CueBench: Advancing Unified Understanding of Context-Aware Video Anomalies in Real-World

How far are deep models from real-world video anomaly understanding (VAU)? Current works typically emphasize on detecting unexpected occurrences deviated from normal patterns or comprehending anomalous events with interpretable descriptions. However, they exhibit only a superficial comprehension of real-world anomalies, with limited breadth in complex principles and subtle context that distinguish the anomalies from normalities, e.g., climbing cliffs with safety gear vs. without it. To this end, we introduce CueBench, the first of its kind Benchmark, devoted to Context-aware video anomalies within a Unified Evaluation framework. We comprehensively establish an event-centric hierarchical taxonomy that anchors two core event types: 14 conditional and 18 absolute anomaly events, defined by their refined semantics from diverse contexts across 174 scenes and 198 attributes. Based on this, we propose to unify and benchmark context-aware VAU with various challenging tasks across recognition, temporal grounding, detection, and anticipation. This also serves as a rigorous and fair probing evaluation suite for generative-discriminative as well as generalized-specialized vision-language models (VLMs). To address the challenges underlying CueBench, we further develop Cue-R1 based on R1-style reinforcement fine-tuning with verifiable, task-aligned, and hierarchy-refined rewards in a unified generative manner. Extensive results on CueBench reveal that, existing VLMs are still far from satisfactory real-world anomaly understanding, while our Cue-R1 surpasses these state-of-the-art approaches by over 24% on average.

==> section/2_Related_Work.tex <==

\section{Related Work}
% \paragraph{Vision-Language Models.}
\noindent \textbf{Vision-Language Models.}
% Discriminative VLMs
The advent of large vision-language models (VLMs) has spurred research in multi-modal contexts, especially in video understanding. With the seminal works such as CLIP [] and ALIGN [] serving as \textit{discriminative VLMs}, have shed light on efficient vision-language alignment for open-vocabulary video applications in action recognition [], action detection [], action anticipation [], anomaly detection [] and etc. 
% Generative VLMs
Recent research interest has shifted towards the development of \textit{generative VLMs} with powerful large language models (LLMs) [] to thrive multi-modal understanding and generation capabilities on captioning [] and question-answering [], as exemplified by as series of groundbreaking commercial models [] like GPT-4o [], Gemini-1.5 [].
The emergence of open-source LLMs [], coupled with progress in multi-modal alignment for vision encoding [], has enabled significant research into public generative VLMs, breeding impressive works such as VideoChat [], Video-LLaMA [], Qwen-VL [] and InternVideo[].
% VAU
With significant achievements in general video understanding, such progresses underscore the need to gauge the capabilities of these VLMs for unified VAU in real-world scenarios.

% \paragraph{Video Anomaly Understanding.}
\noindent \textbf{Video Anomaly Understanding.}
% [Approach-VAD] 
Traditional VAU works primarily focus on VAD settings, with most benchmarks typically restricted to simulate anomalies in the wild [] or to study anomalies within limited real-world scenarios [].
In this direction, VAD approaches have emerged to detect deviations from the learned normal patterns in a semi [] or weakly-supervised [] manner, since anomalous events are scattered and rare occurrences in practice [].
Despite the exploration of semantic information in OVVAD [] or scene-dependencies [] underlying anomalies in NWPU Campus [], a significant gap remains in real-world anomaly understanding with context indispensability [].
% [bench-VAU] 
Building upon the significant achievements of VLMs, the research community has pursued further exploration of VAU benchmarks to probe the multi-modal anomaly understanding abilities with VQA setups of captioning [], causation reasoning [] and user interactions [].
% [anomaly] 
Despite these benchmarks have enriched anomaly dependency from superficial deviations to anomalous events in open-world multi-modalities, they still lag behind the broader understanding of diverse context-dependent anomalies and normalities in real-world.
% [ours]
In response to this need, our \textbf{\cuebench} is the first dedicated to context-aware video anomalies in real-world within a unified evaluation across diverse tasks, marking a significant stride toward more nuanced and comprehensive VAU, as shown in~\tabref{bench}. 
It also features a comprehensive hierarchical taxonomy for absolute and conditional anomalies or normalities, tapping into the underlying refined semantics of scenes and attributes.

% \paragraph{Video Anomaly Understanding with Generative Vision-Language Models.}
\noindent \textbf{Video Anomaly Understanding with Generative Vision-Language Models.}
% 
Recent studies have demonstrated the reliable capabilities of generative vision-language models in VAU. 
Leveraging the exceptional logical reasoning capabilities of VLMs, A-Guardian [] introduces a prompt mechanism to guide VLMs to focus on critical anomaly clues in the video, thus building a logic chain of the cause-effect.
HAWK [] pushes VLM's motion-related interpretation capability of video anomalies by incorporating the motion modality via motion attention reinforcement.
Recently, Holmes-VAU [] proposes the anomaly-focused temporal sampler to reduce the temporal redundancy of VLMs for accurate anomaly detection and understanding in long-term videos.
Unlike these works, we delve into the GRPO-based reinforcement learning from Open-R1 [] and adopts verifiable rewards to perform post-training, this enhancing the VLMs' reasoning capabilities to address the challenges within \cuebench.


==> section/Checklist.tex <==

\newcommand{\answerYes}[1]{\textcolor{blue}{#1}} 
\newcommand{\answerNo}[1]{\textcolor{orange}{#1}} 
\newcommand{\answerNA}[1]{\textcolor{gray}{#1}} 
\newcommand{\answerTODO}[1]{\textcolor{red}{#1}} 
\newcommand{\answerPartial}[1]{\textcolor{teal}{#1}}


\section*{Reproducibility Checklist}

\begin{enumerate}

\item This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)
    
    Answer: \answerYes{[Yes]}
    
  \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)

    Answer: \answerYes{[Yes]}

   \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no)
   
    Answer: \answerYes{[Yes]} 
\end{itemize}

\item Does this paper make theoretical contributions? (yes/no)

Answer: \answerNo{[No]}

% If yes, please complete the list below.
% \begin{itemize}
%   \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)

%     Answer: \answerYes{[Yes]}
    
%   \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)

%     Answer: \answerYes{[Yes]}
    
%   \item Proofs of all novel claims are included. (yes/partial/no)

%     Answer: \answerYes{[Yes]}
    
%   \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)

%     Answer: \answerYes{[Yes]}
    
%   \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
    
%     Answer: \answerYes{[Yes]}
    
%   \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)

%     Answer: \answerYes{[Yes]}
    
%   \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)

%     Answer: \answerYes{[Yes]}
    
% \end{itemize}


\item Does this paper rely on one or more datasets? (yes/no)

Answer: \answerYes{[Yes]}

If yes, please complete the list below.
\begin{itemize}
  \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)
  
    Answer: \answerYes{[Yes]}
    
  \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
  
    Answer: \answerYes{[Yes]}
    
  \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
  
    Answer: \answerYes{[Yes]}
    
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)
    
    Answer: \answerYes{[Yes]}
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)
  
    Answer: \answerYes{[Yes]}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
    
    Answer: \answerYes{[Yes]}

\end{itemize}

\item Does this paper include computational experiments? (yes/no)

Answer: \answerYes{[Yes]}

If yes, please complete the list below.
\begin{itemize}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)

    Answer: \answerYes{[Yes]}

  \item Any code required for pre-processing data is included in the appendix. (yes/partial/no).
    
    Answer: \answerYes{[Yes]}
    
  \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)

    Answer: \answerYes{[Yes]}
    
  \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)
  
    Answer: \answerYes{[Yes]}
    
   \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)
   
   Answer: \answerYes{[Yes]}
   
   If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)

   Answer: \answerYes{[Yes]}
   \item 
This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)

Answer: \answerYes{[Yes]}

\item 
This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)

Answer: \answerYes{[Yes]}

\item 
This paper states the number of algorithm runs used to compute each reported result. (yes/no)

Answer: \answerYes{[Yes]}
\item 
Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)

Answer: \answerYes{[Yes]}
\item 
The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)

Answer: \answerYes{[Yes]}
\item 
This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)

Answer: \answerYes{[Yes]}


\end{itemize}

\end{enumerate}



==> section/ReproducibilityChecklist.tex <==
\makeatletter
\@ifundefined{isChecklistMainFile}{
  % We are compiling a standalone document
  \newif\ifreproStandalone
  \reproStandalonetrue
}{
  % We are being \input into the main paper
  \newif\ifreproStandalone
  \reproStandalonefalse
}
\makeatother

\ifreproStandalone
% \documentclass[letterpaper]{article}
% \usepackage[submission]{aaai2026}
\setlength{\pdfpagewidth}{8.5in}
\setlength{\pdfpageheight}{11in}
% \usepackage{times}
% \usepackage{helvet}
% \usepackage{courier}
% \usepackage{xcolor}
\frenchspacing

% \begin{document}
\fi
\setlength{\leftmargini}{20pt}
\makeatletter\def\@listi{\leftmargin\leftmargini \topsep .5em \parsep .5em \itemsep .5em}
\def\@listii{\leftmargin\leftmarginii \labelwidth\leftmarginii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}
\def\@listiii{\leftmargin\leftmarginiii \labelwidth\leftmarginiii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}\makeatother

\setcounter{secnumdepth}{0}
\renewcommand\thesubsection{\arabic{subsection}}
\renewcommand\labelenumi{\thesubsection.\arabic{enumi}}

\newcounter{checksubsection}
\newcounter{checkitem}[checksubsection]

\newcommand{\checksubsection}[1]{%
  \refstepcounter{checksubsection}%
  \paragraph{\arabic{checksubsection}. #1}%
  \setcounter{checkitem}{0}%
}

\newcommand{\checkitem}{%
  \refstepcounter{checkitem}%
  \item[\arabic{checksubsection}.\arabic{checkitem}.]%
}
\newcommand{\question}[2]{\normalcolor\checkitem #1 #2 \color{blue}}
\newcommand{\ifyespoints}[1]{\makebox[0pt][l]{\hspace{-15pt}\normalcolor #1}}

\section*{Reproducibility Checklist}

% \vspace{1em}
% \hrule
% \vspace{1em}

% \textbf{Instructions for Authors:}

% This document outlines key aspects for assessing reproducibility. Please provide your input by editing this \texttt{.tex} file directly.

% For each question (that applies), replace the ``Type your response here'' text with your answer.

% \vspace{1em}
% \noindent
% \textbf{Example:} If a question appears as
% %
% \begin{center}
% \noindent
% \begin{minipage}{.9\linewidth}
% \ttfamily\raggedright
% \string\question \{Proofs of all novel claims are included\} \{(yes/partial/no)\} \\
% Type your response here
% \end{minipage}
% \end{center}
% you would change it to:
% \begin{center}
% \noindent
% \begin{minipage}{.9\linewidth}
% \ttfamily\raggedright
% \string\question \{Proofs of all novel claims are included\} \{(yes/partial/no)\} \\
% yes
% \end{minipage}
% \end{center}
% %
% Please make sure to:
% \begin{itemize}\setlength{\itemsep}{.1em}
% \item Replace ONLY the ``Type your response here'' text and nothing else.
% \item Use one of the options listed for that question (e.g., \textbf{yes}, \textbf{no}, \textbf{partial}, or \textbf{NA}).
% \item \textbf{Not} modify any other part of the \texttt{\string\question} command or any other lines in this document.\\
% \end{itemize}

% You can \texttt{\string\input} this .tex file right before \texttt{\string\end\{document\}} of your main file or compile it as a stand-alone document. Check the instructions on your conference's website to see if you will be asked to provide this checklist with your paper or separately.

% \vspace{1em}
% \hrule
% \vspace{1em}

% The questions start here

\checksubsection{General Paper Structure}
\begin{itemize}

\question{Includes a conceptual outline and/or pseudocode description of AI methods introduced}{(yes/partial/no/NA)}
yes

\question{Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results}{(yes/no)}
yes

\question{Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper}{(yes/no)}
yes

\end{itemize}
\checksubsection{Theoretical Contributions}
\begin{itemize}

\question{Does this paper make theoretical contributions?}{(yes/no)}
no

	\ifyespoints{\vspace{1.2em}If yes, please address the following points:}
        \begin{itemize}
	
	\question{All assumptions and restrictions are stated clearly and formally}{(yes/partial/no)}
	NA

	\question{All novel claims are stated formally (e.g., in theorem statements)}{(yes/partial/no)}
	NA

	\question{Proofs of all novel claims are included}{(yes/partial/no)}
	NA

	\question{Proof sketches or intuitions are given for complex and/or novel results}{(yes/partial/no)}
	NA

	\question{Appropriate citations to theoretical tools used are given}{(yes/partial/no)}
	NA

	\question{All theoretical claims are demonstrated empirically to hold}{(yes/partial/no/NA)}
	NA

	\question{All experimental code used to eliminate or disprove claims is included}{(yes/no/NA)}
	NA
	
	\end{itemize}
\end{itemize}

\checksubsection{Dataset Usage}
\begin{itemize}

\question{Does this paper rely on one or more datasets?}{(yes/no)}
yes

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

	\question{A motivation is given for why the experiments are conducted on the selected datasets}{(yes/partial/no/NA)}
	yes

	\question{All novel datasets introduced in this paper are included in a data appendix}{(yes/partial/no/NA)}
	yes

	\question{All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no/NA)}
	yes

	\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations}{(yes/no/NA)}
	yes

	\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available}{(yes/partial/no/NA)}
	yes

	\question{All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing}{(yes/partial/no/NA)}
	yes

\end{itemize}
\end{itemize}

\checksubsection{Computational Experiments}
\begin{itemize}

\question{Does this paper include computational experiments?}{(yes/no)}
yes

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

	\question{This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting}{(yes/partial/no/NA)}
	yes

	\question{Any code required for pre-processing data is included in the appendix}{(yes/partial/no)}
	yes

	\question{All source code required for conducting and analyzing the experiments is included in a code appendix}{(yes/partial/no)}
	yes

	\question{All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no)}
	yes
        
	\question{All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from}{(yes/partial/no)}
	yes

	\question{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results}{(yes/partial/no/NA)}
	yes

	\question{This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks}{(yes/partial/no)}
	yes

	\question{This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics}{(yes/partial/no)}
	yes

	\question{This paper states the number of algorithm runs used to compute each reported result}{(yes/no)}
	yes

	\question{Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information}{(yes/no)}
	yes

	\question{The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank)}{(yes/partial/no)}
	yes

	\question{This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments}{(yes/partial/no/NA)}
	yes


\end{itemize}
\end{itemize}
\ifreproStandalone
% \end{document}
\fi
